Palu: Compressing KV-Cache with Low-Rank Projection

Post-training KV-Cache compression methods typically either sample a subset of effectual tokens or quantize the data into lower numerical bit width. However, these methods cannot exploit redundancy in the hidden dimension of the KV tensors. This paper presents a hidden dimension compression approach called Palu, a KV-Cache compression framework that utilizes low-rank projection to reduce inference-time LLM memory usage. Palu decomposes the linear layers into low-rank matrices, caches compressed intermediate states, and reconstructs the full keys and values on the fly. To improve accuracy, compression rate, and efficiency, Palu further encompasses (1) a medium-grained low-rank decomposition scheme, (2) an efficient rank search algorithm, (3) low-rank-aware quantization compatibility enhancements, and (4) optimized GPU kernels with operators fusion. Extensive experiments with popular LLMs show that Palu compresses KV-Cache by 50% while maintaining strong accuracy and delivering up to 1.89x on the RoPE-based attention module. When combined with quantization, Palu's inherent quantization-friendly design yields small to negligible extra accuracy degradation while saving additional memory than quantization-only methods and achieving up to 2.91x speedup for the RoPE-based attention. Moreover, it maintains comparable or even better accuracy (up to 1.19 lower perplexity) compared to quantization-only methods. These results demonstrate Palu's superior capability to effectively address the efficiency and memory challenges of LLM inference posed by KV-Cache. Our code is publicly available at: https://github.com/shadowpa0327/Palu

==> tables/decomposition_overhead.tex <==
\begin{table}[H]
    \caption{
    Numerical analysis on the FLOPs to complete the reconstruction of $\mathbf{y}_i$ for all heads and the size of a fused weight matrix under different decomposition granularity. Here, we assume L = 4096, $n_h$ = 32, $d_h$ = 128, and the total KV-Cache reduction rate to be 50\%.}
\resizebox{20em}{!}{
\begin{tabular}{ c | c | c | c | c }
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{gs} & Reconstruct & Fusion & Fusion \\
                        &                     & (FLOPs)     & (FLOPs) & (\#Params)\\
% 標個倍數(Nx)
\midrule
    Original &  - &     -   &     -   &  16 M \\
    J-LRD    & 32 & 34.38 G & 0.268 G & 256 M \\
    G-LRD    &  4 &  4.31 G & 0.033 G &  32 M \\
    G-LRD    &  2 &  2.16 G & 0.016 G &  16 M \\
    M-LRD    &  1 &  1.09 G & 0.008 G &   8 M \\

\bottomrule
\end{tabular}}
\label{tab:decomposition_overhead}
\end{table}

==> tables/e2e_decoding_latency.tex <==
\begin{table}[!ht]
    \centering
    \caption{End-to-end decoding latency of Llama-2-7B with \palu{} measured on A6000.}
    \resizebox{20em}{!}{
    \begin{tabular}{ l | c | c c c c}
        \toprule
            \multirow{2}{*}{Method} & Group & \multicolumn{4}{c}{Sequence Length} \\
            & Size & 4k & 8k & 16k & 32k \\
        \midrule
            Baseline & - & 36.07 & 44.03 & 69.28 & 112.75 \\
        \midrule
            J-LRD & 32 & 86.39 & 103.41 & 140.85 & OOM \\
            G-LRD &  4 & 32.12 & 38.89 & 52.69 & 80.81 \\
            G-LRD &  2 & 28.82 & 34.94 & 47.45 & 72.89 \\
            M-LRD &  1 & 27.00 & 32.46 & 43.56 & 66.13 \\
        \bottomrule
    \end{tabular}}
    \label{tab:e2e_decoding_latency}
\end{table}


==> tables/llama3_zero_shot.tex <==
\begin{table}[htp]
\centering
\caption{
    Zero-shot accuracy of Palu on LLama3 models. Here, we perform decomposition with a group size of 4. 
}
\resizebox{40em}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{c|l|l|ccccccc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multirow{2}{*}{ \begin{tabular}{@{}c@{}}Comp. \\ Ratio\end{tabular}} & \multicolumn{7}{c}{Zero-Shot Accuracy (\%)\uparrow} \\ 
&  &  & OBQA & Hella & PIQA & ARC-e & ARC-c & Wino & Avg. \\ \midrule
\multirow{5}{*}{Llama3-8b-Instru} & Baseline & 1x & \multicolumn{1}{r}{43.20\%} & \multicolumn{1}{r}{75.80\%} & \multicolumn{1}{r}{78.62\%} & \multicolumn{1}{r}{81.61\%} & \multicolumn{1}{r}{56.83\%} & \multicolumn{1}{r}{71.90\%} & 67.99\% \\  
 & Palu-30\% & 1.43x & \multicolumn{1}{r}{43.60\%} & \multicolumn{1}{r}{75.04\%} & \multicolumn{1}{r}{76.77\%} & \multicolumn{1}{r}{79.42\%} & \multicolumn{1}{r}{54.18\%} & \multicolumn{1}{r}{72.69\%} & 66.95\% \\  
 & Palu-50\% & 2.00x & \multicolumn{1}{r}{42.60\%} & \multicolumn{1}{r}{70.36\%} & \multicolumn{1}{r}{76.06\%} & \multicolumn{1}{r}{76.30\%} & \multicolumn{1}{r}{48.99\%} & \multicolumn{1}{r}{72.38\%} & 64.45\% \\ \cmidrule{2-10} 
 & Palu-30\% + 3bits & 7.59x & \multicolumn{1}{r}{43.80\%} & \multicolumn{1}{r}{73.96\%} & \multicolumn{1}{r}{77.97\%} & \multicolumn{1}{r}{78.37\%} & \multicolumn{1}{r}{53.07\%} & \multicolumn{1}{r}{70.96\%} & 66.36\% \\  
 & Palu-50\% + 3bits & 10.6x & \multicolumn{1}{r}{41.20\%} & \multicolumn{1}{r}{69.43\%} & \multicolumn{1}{r}{76.17\%} & \multicolumn{1}{r}{74.83\%} & \multicolumn{1}{r}{46.59\%} & \multicolumn{1}{r}{70.25\%} & 63.08\% \\ \midrule
\end{tabular}
}
\end{table}

==> tables/llama_zero_shot_30.tex <==
\begin{table*}[htp]
\centering
    \caption{
        Zero-shot accuracy of Palu on LLama2 models, with different decomposition strategies at 30\% compression rate.
    }
\resizebox{34em}{!}{
\begin{tabular}{c | l | cccccccc}
\toprule
\multirow{2}{*}{Model}      & \multicolumn{1}{c|}{\multirow{2}{*}{Method}}                                                & \multicolumn{7}{c}{Zero-Shot Accuracy (\%) $\uparrow$}     \\
                            & \multicolumn{1}{c|}{}                                                                        & OBQA  & Hella & PIQA  & ARC-e & ARC-c & Wino  & Avg. & Diff. \\ \midrule
\multirow{4.5}{*}{Llama2-7B}  & Baseline                                                                                     & 44.20 & 76.00 & 78.07 & 76.30 & 46.42 & 69.30 & 65.05 & - \\ \cmidrule{2-10} 
                            & J-LRD                                                                                        & 44.40 & 76.01 & 77.75 & 76.01 & 45.31 & 69.38 & 64.81 & -0.24 \\
                            & G-LRD                                                                                       & 45.20 & 76.07 & 78.56 & 75.93 & 44.97 & 68.75 & 64.91 & -0.14 \\
                            & M-LRD                                                                                        & 43.20 & 73.50 & 77.42 & 74.16 & 42.58 & 68.90 & 63.29 & -1.76 \\ \midrule
\multirow{4.5}{*}{Llama2-13B} & Baseline                                                                                    & 45.20 & 79.39 & 79.11 & 79.42 & 49.06 & 72.38 & 67.43 & - \\ \cmidrule{2-10} 
                            & J-LRD                                                                                        & 45.20 & 79.58 &	80.57&	79.67&	49.40&	71.74&	67.69&  +0.26\\
                            & G-LRD                                                                                        & 46.60 &	79.04 &	78.23&	79.42 &	48.38 &	71.59 &	67.21&	-0.22 \\
                            & M-LRD                                                                                        & 45.40 &	78.57 &	78.78&	78.83 &	47.61 &	72.06 &	66.88&	-0.55  \\ \bottomrule
\end{tabular}
}
\label{tab:llama_zero_shot_30}
\end{table*}


==> tables/longbench.tex <==
\begin{table*}[hbt]
\centering
\caption{Accuracy of \palu{} with 30\% and 50\% compression rate on 8 tasks in LongBench.}
\resizebox{37em}{!}{
\begin{tabular}{c l ccccccccc}
    \toprule
        Model & \multicolumn{1}{c}{Method} & SAMSum & LCC & M-News & Qasper & TREC & QmSum & R-Bench & TriQA & Avg. \\
    \midrule
    \multirow{3.5}{*}{Vicuna-7B}
        & Baseline & 40.73  & 49.20 & 27.98  & 25.57  & 69.00 & 22.54 & 43.50 & 86.42 & 45.62  \\ 
    \cmidrule{2-11} 
        & Palu-30\% & 40.42  & 49.00 & 26.96  & 18.54  & 65.50 & 21.78 & 45.77 & 85.22 & 44.15  \\
        & Palu-50\% & 38.36  & 34.59 & 24.78  & 19.77  & 63.50 & 21.44 & 35.42 & 79.74 & 39.70  \\
    \midrule
    \multirow{3.5}{*}{Mistral-7B} 
        & Baseline & 41.71  & 66.59 & 20.26  & 8.13   & 67.00 & 19.99 & 59.10 & 89.90 & 46.59  \\ \cmidrule{2-11}
        & Palu-30\% & 43.23  & 64.23 & 23.50  & 10.21  & 72.50 & 21.16 & 56.80 & 89.82 & 47.68  \\
        & Palu-50\%  & 36.43  & 50.22 & 19.23  & 7.54   & 67.50 & 19.56 & 44.76 & 85.37 & 41.33  \\
    \bottomrule
\end{tabular}}
\label{tab:longbench}
\end{table*}

==> tables/quantization.tex <==
\begin{table}[tbh!]
\caption{Perplexity and \kv{} size comparison of \palu{} and other quantization-based methods for Llama2-7B on WikiText-2. For perplexity, sequence length is set to 4096, aligning with baselines. \kv{} size is demonstrated for a sequence length of 128K. % For \palu{}, we use G-LRD with group size 4.
% \chienyu{New version with \kv{} size back but without the compression rate to Atom. We can compare with previous version and decide which is better.}
}
\centering
\resizebox{17em}{!}{
\begin{tabular}{ l | c | c | c | c }
        \toprule
        Method & Bit & PPL &  \begin{tabular}{@{}c@{}}\kv{} \\ Size (GB) \end{tabular} & \begin{tabular}{@{}c@{}}Comp. \\ Rate \end{tabular} \\
        
        \midrule
        Baseline         & 16 & 5.12  & 64.0 & -      \\
        \cmidrule{1-5} 
        Palu-30\%        & 16 & 5.25  & 44.8 & 30\%   \\ 
        Palu-50\%        & 16 & 5.63  & 32.0 & 50\%   \\
        \cmidrule{1-5}         
        Atom             & 3  & 6.15  & 12.6 & 80.32\% \\
        KVQuant          & 3  & 5.35  & 12.0 & 81.25\% \\
        Palu-30\%        & 3  & \textbf{5.33}  & \textbf{8.4}  & \textbf{86.87\%} \\
        Palu-50\%        & 3  & 5.77  & 6.0  & 90.63\% \\
        \cmidrule{1-5}
        Atom             & 2 & 117.88 & 8.6  & 86.56\% \\
        KVQuant          & 2 &   6.95 & 8.0  & 87.50\% \\
        Palu-30\%        & 2 & \textbf{5.76} & \textbf{5.6} & \textbf{91.25\%} \\
        Palu-50\%        & 2 & \textbf{6.41} & \textbf{4.0} & \textbf{93.75\%} \\
        \bottomrule
\end{tabular}}
\label{tab:quantization}
\end{table}

==> tables/zero_shot_results_old_.tex <==
\begin{table*}[hbt]
\centering
\caption{Evaluation of Palu for Llama2-7B on six common sense zero-shot tasks. 
% The results of Mistrial-7B Is at \ref{}
}
\resizebox{37em}{!}{
\begin{tabular}{ l | l | c  cccccccc }
\toprule
Comp. Rate & Method & OBQA & HellaSwag & PIQA & ARC-e & ARC-c & WinoGrande & Avg. & Diff. \\

\midrule

 Ratio = 0\% & baseline        & 44.20 & 76.00 & 78.07 & 76.30 & 46.42 & 69.30 & 65.05 & - \\
\midrule
\multirow{3}{*}{\begin{tabular}{@{}l@{}}Ratio = 50\%\\ w/o LoRA  \end{tabular}}
& J-LRD        & 45.20 & 74.61 & 77.04 & 74.58 & 44.20 & 69.53 & 64.19 & -0.85 \\
& G-LRD (gs=4) & 37.80 & 69.64 & 73.39 & 67.09 & 37.37 & 65.43 & 58.45 & -6.60 \\
& M-LRD        & 38.40 & 64.41 & 73.23 & 65.74 & 35.49 & 60.77 & 56.34 & -8.71 \\
\midrule
\multirow{3}{*}{\begin{tabular}{@{}l@{}}Ratio = 50\%\\ w/ LoRA  \end{tabular}}
& J-LRD         & 43.40 & 74.75 & 77.86 & 74.49 & 44.28 & 69.53 & 64.05 & -1.00 \\
& G-LRD (gs=4)  & 44.20 & 71.62 & 77.97 & 72.56 & 44.03 & 68.19 & 63.10 & -1.95 \\
& M-LRD         & 41.00 & 69.65 & 76.82 & 72.69 & 42.32 & 67.01 & 61.58 & -3.47 \\

\bottomrule
\end{tabular}}
\label{tab:zero_shot_results}
\end{table*}
